Rescaling-Aware Training for Efficient Deployment of Deep Learning Models on Full-Integer Hardware

Integer AI inference significantly reduces computational complexity in embedded systems. Quantization-aware training (QAT) helps mitigate accuracy degradation associated with post-training quantization but still overlooks the impact of integer rescaling during inference, which is a hardware costly operation in integer-only AI inference. This work shows that rescaling cost can be dramatically reduced post-training, by applying a stronger quantization to the rescale multiplicands at no model-quality loss. Furthermore, we introduce Rescale-Aware Training, a fine tuning method for ultra-low bit-width rescaling multiplicands. Experiments show that even with 8x reduced rescaler widths, the full accuracy is preserved through minimal incremental retraining. This enables more energy-efficient and cost-efficient AI inference for resource-constrained embedded systems.

==> figures/tikz/rescaling-unit.tex <==
\begin{tikzpicture}[
    >={Stealth[round]},                     
    every node/.style={font=\small},
    % ------------------------------------------------------------------
    % base styles
    % ------------------------------------------------------------------
    baseblock/.style={draw, rectangle, rounded corners=2pt,
                      inner sep=0pt},
    int/.style={baseblock, minimum width=0.5cm, minimum height=0.5cm,
                fill=blue!15},
    bigblock/.style={baseblock, rounded corners=4pt, inner sep=3pt,
                     minimum width=2cm, minimum height=1.3cm,
                     fill=green!10, draw=green!80!black, line width=0.1mm},
    smallblock/.style={baseblock, minimum width=1.4cm, minimum height=0.8cm,
                       fill=yellow!30},
    grayblock/.style={baseblock, minimum size=0.5cm, inner sep=3pt, fill=gray!15},
    tiny/.style={baseblock, minimum size=0.5cm, fill=gray!20},
    % arrow styles
    arrow8/.style={->},
    arrow32/.style={->, line width=1pt},
    arrow64/.style={->, line width=2pt}
]

% ----------------------------------------------------------------------
% 1)  Outer “Operation” block (container, in background)
% ----------------------------------------------------------------------
\begin{pgfonlayer}{background}
    \node[bigblock, minimum height=1.95cm, minimum width=2.1cm] (operation) {};
\end{pgfonlayer}
\node[anchor=north] at (operation.north) {\bfseries Operation};

% ----------------------------------------------------------------------
% 2)  Quantised inputs (on the left, stacked vertically)
% ----------------------------------------------------------------------
\node[int, above=0.7cm of operation.north, xshift=-0.6cm] (xq) {$\mathbf{x}_q$};
\node[int, above=0.7cm of operation.north, xshift= 0.6cm] (wq) {$\mathbf{w}_q$};

\draw[arrow8] (xq.south) -- node[midway,yshift=0.1cm,font={\scriptsize},fill=white] {$\texttt{int8}$} (xq |- operation.north);
\draw[arrow8] (wq.south) -- node[midway,yshift=0.1cm,font={\scriptsize},fill=white] {$\texttt{int8}$} (wq |- operation.north);

% ----------------------------------------------------------------------
% 3)  Accumulator block (inside "Operation")
% ----------------------------------------------------------------------
\node[grayblock, above=0.2cm of operation.south, minimum width=1.5cm] (accumulator) {\textit{Accumulator}};
\node[grayblock, above=0.2cm of accumulator.north, minimum width=1.5cm] (Mac) {\textit{MACs}};

% ----------------------------------------------------------------------
% 4)  Rescaling container
% ----------------------------------------------------------------------
\begin{pgfonlayer}{background}
    \node[draw, bigblock, line width=0.4mm,
    right=0.9cm of operation, yshift=-0.3cm, 
    minimum width=4.28cm, minimum height=1.3cm,
    fill=yellow!20, draw=yellow!90!black] (rescale) {};
\end{pgfonlayer}
\node[anchor=north east, xshift=-0.45cm] at (rescale.north east) {\bfseries Rescaling};

% ----------------------------------------------------------------------
% 5)  Rescaling symbols
% ----------------------------------------------------------------------
% , below right=0.2cm of rescale.north west
\node[tiny, anchor=north west, xshift=0.2cm] (mult) at (rescale.west |- accumulator.north) {$\times$};
\node[tiny, right=0.9cm of mult] (shft) {$\gg$};
\node[grayblock, right=0.9cm of shft] (saturation) {\textit{Clamp}};

% ----------------------------------------------------------------------
% 6)  Rescale-parameter block (above rescale)
% ----------------------------------------------------------------------
\node[smallblock, fill=orange!20, draw=orange!80!black, line width=0.1mm,
    anchor=north west, minimum width=2.18cm] (rescale_param)
      at (rescale.west |- xq.north)
      {$M_q = \dfrac{m}{2^{s}}$};

\draw[arrow32] (mult.north |- rescale_param.south) -- (mult.north)
      node[midway,yshift=0.2cm,font={\scriptsize},fill=white] {$\texttt{int32}$};
\draw[arrow8] (shft.north |- rescale_param.south) -- (shft.north);

% ----------------------------------------------------------------------
% 7)  Remaining connections
% ----------------------------------------------------------------------
%\draw[arrow8] (Mac) -- (accumulator);
\draw[arrow8] (Mac) -- (accumulator);
\draw[arrow8] ($ (Mac.south) + (-0.4,0) $) -- ($ (accumulator.north) + (-0.4,0) $);
\draw[arrow8] ($ (Mac.south) + (0.4,0) $) -- ($ (accumulator.north) + (0.4,0) $);

\draw[arrow32] (accumulator.east) -- node[midway,above,font={\scriptsize}] {$\texttt{int32}$} (mult.west);
\draw[arrow64] (mult) -- node[midway,above,font={\scriptsize},color=black] {$\texttt{int64}$} (shft);

\draw[arrow32] (shft.east) -- node[midway,above,font={\scriptsize}] {$\texttt{int32}$} (saturation.west);

\node[int, right=0.9cm of rescale] (yq) at (rescale.east |- saturation.east) {$\mathbf{y}_q$};
\draw[arrow32] (saturation) -- node[midway,above,font={\scriptsize}] {$\texttt{int8}$} (yq);

\end{tikzpicture}

